Tutorial: Object as a Service (OaaS) Serverless Cloud Computing Paradigm

While the first generation of cloud computing systems mitigated the job of system administrators, the next generation of cloud computing systems is emerging to mitigate the burden for cloud developers -- facilitating the development of cloud-native applications. This paradigm shift is primarily happening by offering higher-level serverless abstractions, such as Function as a Service (FaaS). Although FaaS has successfully abstracted developers from the cloud resource management details, it falls short in abstracting the management of both data (i.e., state) and the non-functional aspects, such as Quality of Service (QoS) requirements. The lack of such abstractions implies developer intervention and is counterproductive to the objective of mitigating the burden of cloud-native application development. To further streamline cloud-native application development, we present Object-as-a-Service (OaaS) -- a serverless paradigm that borrows the object-oriented programming concepts to encapsulate application logic and data in addition to non-functional requirements into a single deployment package, thereby streamlining provider-agnostic cloud-native application development. We realized the OaaS paradigm through the development of an open-source platform called Oparaca. In this tutorial, we will present the concept and design of the OaaS paradigm and its implementation -- the Oparaca platform. Then, we give a tutorial on developing and deploying the application on the Oparaca platform and discuss its benefits and its optimal configurations to avoid potential overheads.

==> src/availability.tex <==

\section{Oparaca Code and Resource Availability}
The source code of Oparaca is publicly available at the following GitHub repository: \url{https://github.com/hpcclab/OaaS}  
This repository includes the document for deploying the Oparaca to the Kubernetes cluster and some example applications to be deployed on Oparaca.

==> src/biography.tex <==
\section{Biography of the instructor(s)}
\label{sec:biography}
Dr. Mohsen Amini Salehi is an Associate Professor at the Computer Science and Engineering (CSE) department, University of North Texas (UNT), USA. He is the director of High Performance and Cloud Computing (HPCC) Laboratory where several graduate and undergraduate students research on various aspects of Distributed and Cloud computing. Dr. Amini is an NSF CAREER Awardee and, so far, he has had 11 research projects funded by National Science Foundation
(NSF) and Board of Regents of Louisiana. He has
also received 10 awards and certificates from in recognition of his innovative research, including the “Best Service Award” from IEEE/ACM CCGrid '23 Conference. His research interests are in democratizing cloud-native application development, building smart and trustworthy systems across edge-to-cloud continuum, and heterogeneous computing.

Pawissanutt Lertpongrujikorn is currently a Ph.D. Student in computer science and engineering at the University of North Texas. Pawissanutt works as a research assistant at the High-Performance Cloud Computing (HPCC) Lab in the computer science and engineering department. His research
interest includes developing a new paradigm for cloud-native programming and serverless systems.
He earned a B.Eng. in computer engineering
from Kasetsart University in Thailand.

==> src/potential.tex <==
\section{Potential Audience of the Tutorial}
\label{sec:potencial}
% LIMIT 100 WORDS

Embracing the OaaS paradigm can benefit developers of small companies or startups trying to develop and deploy new services without bearing the burden of low-level details. By leveraging this paradigm, developers can focus on high-level application logic while offloading the operational aspects of the service to software automation. This results in a more agile and effective development process, which can help startups quickly deliver new services to the market. The company also benefits from a serverless auto-scaling feature, which reduces resource waste during low workloads and maintains user experience during high traffic by dynamically adjusting allocated resources.

% There is a possibility that cloud providers may find \sysname useful to incorporate the OaaS paradigm as an extra development option for their own users. As mentioned earlier, \sysname is designed to be platform-independent, which makes it uncomplicated to integrate with their own solutions.

% \section{Requirements for the Tutorial}

% For this tutorial, we need a projector and internet access for the presenter and audience.
% Audiences who want to follow the tutorial should have some basic knowledge of cloud and Kubernetes and have a laptop that can install container runtime.

% To make the hands-on tutorial flow smoothly, the audience should have a laptop that already installs the basic software requirements: Docker~\cite{merkel2014docker}, Java~\cite{java} (version 21), and Python~\cite{python} (version $>$= 3.11) runtime. Moreover, the laptop should have at least 16 GB of memory to run all of the software without the out-of-memory error.


==> src/toc.tex <==
\section{Table of Contents}

The table of contents of the tutorial will be as follows:

% \begin{enumerate}
%     \item Introduction: Serverless system
%     \item Motivation: The shortages of FaaS and the improvements to the ideal platform 
%     \item Object as a Service (OaaS) Paradigm
%     \item Oparaca Concepts and Designs 
%     \begin{enumerate}
%         \item System Architecture
%         \item Dynamic Class Runtime
%         \item State Management
%         \item Maintaining Consistency with \textit{fail-safe state transition}
%         \item Performance improvement with cashing and consistent hashing
%         \item Dataflow abstraction
%         \item QoS-driven optimization
%     \end{enumerate}
%     \item Demonstration of developing services with Oparaca
%     \begin{enumerate}
%         \item Creating a new function with Python code
%         \item Defining a new class in YAML
%         \item Using Oparaca CLI to manage the class deployment
%         \item Creating a new object and invoking its function
%         \item Optimizing by defining the QoS requirements and constraints
%     \end{enumerate}
        
% \end{enumerate}


\begin{enumerate}
    \item Introduction: 
    \begin{enumerate}
        \item Serverless system and our vision of the next-generation cloud computing.
        \item The current state of the practice, FaaS paradigm 
    \end{enumerate}
    \item Motivations: 
    \begin{enumerate}
        \item The shortages of FaaS 
        \item The problems of guaranteeing application performance in FaaS development.
    \end{enumerate}
    \item Our solutions: Object as a Service (OaaS) Paradigm
    \begin{enumerate}
        \item Unified OaaS Abstraction (Data, function, non-functional requirement encapsulation into the notion of object)
        \item High-level non-functional requirement interface to drive the cloud-developer coordination
    \end{enumerate}
    \item Oparaca Concepts and Designs:
    \begin{enumerate}
        \item Our design goals for designing Oparaca
        \item System Architecture
        \item Dynamic Class Runtime
        \item Requirement-driven optimization
        \item State Management
        \item Maintaining Consistency with \textit{fail-safe state transition}
        \item Performance improvement with caching and consistent hashing via distributed hash table (DHT)
        % \item Dataflow abstraction
    \end{enumerate}
    \item Demonstration of developing services with Oparaca
    \begin{enumerate}
        \item Installing Oparaca platform inside local Kubernetes
        \item Creating a new function with Python code
        \item Defining a new class in YAML
        \item Using Oparaca CLI to manage the class deployment
        \item Creating a new object and invoking its function
        \item Optimizing by defining the non-functional requirement (QoS and constraints)
    \end{enumerate}
\end{enumerate}
